Disentangling the Black Hole Mass Spectrum with Photometric Microlensing Surveys

From the formation mechanisms of stars and compact objects to nuclear physics, modern astronomy frequently leverages surveys to understand populations of objects to answer fundamental questions. The population of dark and isolated compact objects in the Galaxy contains critical information related to many of these topics, but is only practically accessible via gravitational microlensing. However, photometric microlensing observables are degenerate for different types of lenses, and one can seldom classify an event as involving either a compact object or stellar lens on its own. To address this difficulty, we apply a Bayesian framework that treats lens type probabilistically and jointly with a lens population model. This method allows lens population characteristics to be inferred despite intrinsic uncertainty in the lens-class of any single event. We investigate this method's effectiveness on a simulated ground-based photometric survey in the context of characterizing a hypothetical population of primordial black holes (PBHs) with an average mass of $30 M_{\odot}$. On simulated data, our method outperforms current black hole (BH) lens identification pipelines and characterizes different subpopulations of lenses while jointly constraining the PBH contribution to dark matter to ${\approx}25$\%. Key to robust inference, our method can marginalize over population model uncertainty. We find the lower mass cutoff for stellar origin BHs, a key observable in understanding the BH mass gap, particularly difficult to infer in our simulations. This work lays the foundation for cutting-edge PBH abundance constraints to be extracted from current photometric microlensing surveys.

==> scratch.tex <==
%\usepackage{aas_macros}
%\usepackage[linktocpage,breaklinks]{hyperref}

%\hypersetup{colorlinks=true,
%            citecolor=Black,
%            linkcolor=Black,
%            urlcolor=Black}

%\usepackage{mathtools}
%\usepackage{verbatim}
%\usepackage{amssymb}
%\usepackage{amsfonts}
%\usepackage{txfonts}
%\usepackage{bm}
%\usepackage{stmaryrd}
%\usepackage{tensor}
%\usepackage{mathrsfs}
%\usepackage[utf8]{inputenc}
%\usepackage{url}
%\usepackage{booktabs}
%
%\usepackage{epsfig}
%\usepackage{epstopdf}
%\usepackage[normalem]{ulem}
%
%\usepackage{natbib}
%\usepackage{cleveref}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newcommand{\hypshapei}{\boldsymbol{\lambda_i}}
%\newcommand{\hypshapej}{\boldsymbol{\lambda_j}}
%\newcommand{\hypshapek}{\boldsymbol{\lambda_k}}
%\newcommand{\paramvec}{\boldsymbol{\theta} }
%\newcommand{\paramvecprime}{\boldsymbol{\theta \sp{\prime}} }
%\newcommand{\popvec}{ \boldsymbol{\lambda} }
%\newcommand{\popvecprime}{ \boldsymbol{\lambda\sp{\prime}} }
%\newcommand{\class}{{\rm class}_j }
%\newcommand{\classk}{{\rm class}_k }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%\begin{comment}
%Intro 
%	- Why should we care about black holes?
%		- Astrophysics and fundamental physics (DM, PBH, stellar collapse and death)
%		- Existing approaches (with shortfalls)
%			- GW
%			- EHT
%			- Accretion
%	- Why is it hard to detect black holes and do population statistics?
%		- Don't emit except in binaries or accreting  
%	- How can microlensing help?
%		- Microlensing gives us
%			- isolated blackholes
%			- environment 
%		- acknowledge ways to break degeneracy
%				- astrometric + photometric
%					- Lu
%				- What about just photometric?
%				- Maybe mention GAIA
%				- But are EXPENSIVE
%					- Low numbers
%		- Benefits of Photometric mircolensing + statistics
%			- What differentiates black holes from other lensing objects with photometric lensing?
%Summary of paralensing modeling and how \lamspace space measurements can provide information about lenses and underlying lens-population hyperparameters
%	- Define $t_E$, $\theta_E$, $\pi_E$, $\pi_{\rm rel}$
%	- Mass distribution and spatial distribution map to different distributions in \lamspace
%Statistics framework - Selection effects and noisy measurements in Bayesian inference	
%	- Single event analysis
%		- Individual event posteriors on model parameters
%		- Individual source classification (Bayes factor calc)
%	- Population analysis (abridged)
%		- Full framework
%		- Fixed model, mixing fractions
%Verification framework 
%	- What population model do we use? 
%	- How do we construct the sensitivity curves? 
%	- How do we calculate detection efficiency for the population model? 
%	- How do we construct synthetic surveys? 
%	- How do we construct source distributions predictions from a population model? 
%	- How do we calculate the posteriors?
%Application to individual events (source classification)
%	- Can we robustly and semi-confidently detect BHs in the data through sheer photometry with current data?
%	- How can this be used with future surveys for follow up?
%		- How does this change as the signal progresses?
%			- Note, this will change the detection efficiency and population slightly, as the longer integration time changes the sensitivity of the survey 
%Application to fixed population model 
%	- Fit KDE to simulation by class
%	- Take MCMC samples and evaluate probability of each class at each sample (Write out math that this corresponds to (model selection/bayes factors)
%	- Sum and normalize these probabilities to determine probability of each class 
%		- A) by source
%		- B) for overall rates
%Application to flexible population model
%First application to OGLE data
%	- Any confident, single sources?
%	- Mixing fraction?
%Conclusions
%	Systematics that need to be understood
%	Use cases, applications and discussions
%		- Massive Jupiters
%\end{comment}


\begin{comment}
We first turn our focus to the task of ``semi-hierarchical'' inference. 
We use the term semi-hierarchical to denote this type of analysis because we will not be inferring any information about the population itself (therefore, strictly speaking, this is \emph{not} hierarchical), but this analysis will enable us to understand an event in the context of the population it belongs to.
We will continue denoting the existence or non-existence of triggers in the data for completeness, but as we shall soon see, selection effects are still absent as we are still only considering single events.
\sepc{Yes, PopSyCLE has selection cuts, which we will need to relax to effectively be zero. But the analysis, fundamentally, does not incorporate selection effects (or at least it shouldn't).}
We would like to know, given some overall (and comprehensive) population model parameterized by $\hyp$: what is the probability of a single event to belong to a subcategory of the population?
For example, one might be searching for exotic events in the presence of other, more mundane detections, like searching for new particles in particle accelerators, identifying the constituent objects in gravitational wave signals, or in our current situation, identifying whether a microlensing signal was produced by a black hole or a star.

In this situation, we will assume we have some set of classes $\{\classa\}$ with $a\in\{1..\nclass\}$, where $\nclass$ is the number of subpopulations being considered.
Furthermore, we will assume that this is a complete set, i.e., that all sources fall into one of these classes.
In mathematical language, we would like to know the following,
\begin{equation}
p(\classa | \D, \trig, \hyp)
\end{equation}
for some data $\D$ and associated trigger $\trig$.
This means we can use Bayes' theorem to write 
\begin{equation}
p(\classa | \D, \trig, \hyp)= \frac{p(\classa| \hyp)p(\D , \trig | \classa, \hyp)}{p(\D, \trig | \hyp)}\,.
\end{equation}
The prior $p(\classa | \hyp)$ is up to the experimenter (as always), but simply describes the prior probability of a lens to belong to a given class without considering the data yet. 
If a class is expected to make up $90\%$ of the total events, this would be $0.9$, for example. 
\sepc{I mean the total number of events, detected or not. This distribution is \emph{not} conditioned on detection. We do need to define what an event is, however. To keep things reasonable, we can define this as the edge of being able to detect things at all (like a max $u_0$ cut, for example). Not every BH counts as an ``event'', but every BH that passes within XYZ mas of a background source does count, for example.}

We now turn to the likelihood, which we will first transform using the product rule (again, to separate the existence of a trigger from the actual set of data)
\begin{align}\nonumber
p(\D , \trig | \classa, \hyp) = &p(\D | \classa, \hyp) \\
&\times p (\trig | \D , \classa, \hyp) \,,
\end{align}
Noting that, again, the existence of a trigger is only dependent on the data, $p (\trig | \D , \classa, \hyp)= p (\trig | \D )=1$.
This leaves us with the following posterior
\begin{equation}
p(\classa | \D, \trig, \hyp)= \frac{p(\classa| \hyp)p(\D | \classa, \hyp)}{p(\D, \trig | \hyp)}\,.
\end{equation}
Now, to calculate the probability of seeing data $\D$ given some model of a class of sources $\classa$, we need to introduce actual event modeling parameters. 
The $\classa$ hypothesis defines a distribution of the model parameters for a specific class, but does not give us a prediction of the data.
To do that, we can introduce the model parameters into the likelihood and marginalize over them,
\begin{align}\nonumber
p(\D | \classa, \hyp) &= \int p(\D , \eparam | \classa, \hyp) d\eparam \,,\\\nonumber
&=\int p(\D | \eparam , \classa, \hyp) p(\eparam |\classa, \hyp)d\eparam \,,\\
&= \int p(\D | \eparam ) p(\eparam |\classa, \hyp)d\eparam \,,
\end{align}
where we have used marginalization, then the product rule.
We have also used the fact that the data \emph{only depends on the model parameters $\eparam$}, once the likelihood of $\D$ has been conditioned on a specific set of event parameters.
Once event parameters $\eparam$ have been specified, the likelihood of the data is not directly dependent on the population model $\hyp$ or $\classa$.
This gives the following result for the posterior probability of an event belonging to a class 
\begin{align}\label{eq:finalPosteriorclass}\nonumber
p(\classa | \D, \trig, \hyp) &= \frac{p(\classa| \hyp)}{p(\D, \trig | \hyp)} \\
&\times \int p(\D | \eparam ) p(\eparam |\classa, \hyp)d\eparam \,,
\end{align}
where we simply average the likelihood from the single event analysis with the new population prior.
If one wants to reuse discrete samples already drawn from the single event posterior on the event parameters (as is frequently the case~\citep{2010ApJ...725.2166H}), one can start by identifying 
\begin{align}\nonumber
p(\D | \eparam) &= p(\D, \trig | \eparam, \hyp) \,,\\\nonumber
&= \frac{p(\eparam|\D, \trig, \hyp)\pi(\D, \trig| \hyp) }{\pi(\eparam| \hyp)}  \,,\\
&= \frac{p(\eparam|\D,  \hyp)\pi(\D| \hyp) }{\pi(\eparam| \hyp)}\,,
\end{align} 
where we have reintroduced $\hyp$ and $\trig$ hypotheses for clarity, to connect with the above sections.
We also denote the prior and evidence in the original analysis as $\pi(\eparam|\hyp)$ and $\pi(\D |\hyp)$ to avoid confusion with the updated population model.
If samples were drawn from the posterior distribution $p(\eparam|\D,\trig, \hyp)$ in a previous analysis (for example through MCMC sampling), one can approximate the integral over source parameters in Eq.~\eqref{eq:finalPosteriorclass} with Monte Carlo integration
\begin{subequations}
\begin{align}\nonumber
\int p(\D | \eparam ) &p(\eparam |\classa, \hyp)d\eparam \approx \frac{1}{S} \\
&\times \sum_{c=0}^{S} \frac{ p(\eparamc |\classa, \hyp)\pi(\D| \hyp)}{\pi(\eparamc| \hyp)}\,,
\end{align}
\begin{equation}
\eparamc \sim p(\eparam | \D, \trig, \hyp) \,,
\end{equation}
\end{subequations}
where $S$ is the number of samples for event posterior for the event. 

Putting all of this together, one gets
%\begin{empheq}[box=\fbox]{align}\label{eq:class_post}\nonumber
\begin{align}\label{eq:class_post}\nonumber
p(\classa | \D, \trig, \hyp) \approx  &\frac{p(\classa| \hyp)\pi(\D| \hyp)}{p(\D, \trig | \hyp)}\\
&\times \frac{1}{S} \sum_{c=0}^{S} \frac{ p(\eparamc |\classa, \hyp)}{\pi(\eparamc| \hyp)} \,.
\end{align}
%\end{empheq}
This framework of source classification is also consistent with viewing this challenge as a model selection problem, as the integral over the event posterior is simply the evidence for an event conditioned on $\classa$. 
This yields the expected Bayes' factor expression for the probability between two classes for a single event
\begin{align}\nonumber
\mathcal{O}_{a,b} &= \frac{p(\classa | \D , \trig, \hyp)}{p(\classb | \D , \trig, \hyp)} \,,\\\nonumber
&= \frac{p(\classa| \hyp)}{p(\classb| \hyp)} \frac{\int p(\D | \eparam ) p(\eparam |\classa, \hyp)d\eparam}{\int p(\D | \eparam ) p(\eparam |\classb, \hyp)d\eparam}\,,\\\nonumber
&=\frac{p(\classa| \hyp)}{p(\classb| \hyp)} \frac{ p(\D |\classa, \hyp)}{p(\D |\classb, \hyp)}\,,\\
&=\frac{p(\classa| \hyp)}{p(\classb| \hyp)} \mathcal{B}_{a,b}\,,
\end{align}
where the first line uses the definition of $p(\classa | \D, \trig, \hyp)$ of Eq.~\eqref{eq:finalPosteriorclass}, and $\mathcal{B}_{a,b}$ is the traditional Bayes' factor in favor of model $a$ over $b$.

Taking this one step further, we can write out the (normalized) posterior probability of a single lens belonging to a specific class, $\classa$, as we can calculate the necessary normalization constant by noting that we are currently assuming a finite and complete number of classes.
We must simply note that
\begin{equation}
p(\D, \trig | \hyp) = \sum_b p(\classb|\hyp) p(\D,\trig|\classb, \hyp)\,,
\end{equation}
where we can now rewrite Eq.~\eqref{eq:finalPosteriorclass} as a normalized probability density, giving
\begin{equation}
p(\classa | \D, \trig, \hyp) = \frac{p(\classa | \hyp) p(\D, \trig | \classa, \hyp)}{\sum_b p(\classb|\hyp) p(\D,\trig|\classb, \hyp)}\,.
\end{equation}

\end{comment}

\begin{comment}
\subsection{Population Analysis}\label{sec:populations}
% Define pdet and alpha
Before extending the above analysis to a full hierarchical framework, we will define a few key quantities below. 
Namely, the two distributions $p(\trig| \hyp)$ and $p(\trig|\eparam)$, which identically canceled above. 
As we will see below, these do not cancel for hierarchical population analyses and must be calculated.
To begin, we will focus on $p(\trig|\eparam)$, which is the probability of a trigger given a source exists with a certain set of parameters $\eparam$.
As the concept of a trigger is inherently tied to detector noise and detector limitations, we will need to introduce a set of data $\D$ as a parameter and marginalize over all possible noise realizations.
\begin{align}\nonumber
p(\trig|\eparam) &= \int p(\trig , \D | \eparam)\;d\D \,,\\\nonumber
 &= \int p(\trig | \D , \eparam) p(\D|\eparam)\;d\D\,,\\
 &= \int  p(\trig | \D ) p(\D|\eparam)\;d\D\,,
\end{align}
where we have used the fact that once a noise realization is measured, the probability of a trigger conditioned on that data \emph{only} depends on the data itself.
The quantity $p(\D| \eparam)$ is simply the likelihood of the single-event analysis, which is another way of specifying the noise model of the detector. 
So this ends up being the average of $p(\trig|\D)$ weighted against the expected noise realizations $p(\D| \eparam)$.
This can be evaluated with various methods. 
For example, one can inject fake signals into detection pipelines and record the different numbers of detections and non-detections, which is a certain form of Monte Carlo integration.
We can always evaluate the above integral with 
\begin{subequations}\label{eq:pdet}
\begin{equation}
p(\trig| \eparam) \approx \frac{1}{S}\sum_{c = 0}^S p(\trig| \Dc)\,,
\end{equation}
\begin{equation}
\Dc \sim p(\D|\eparam)\,,
\end{equation}
\end{subequations}
given $S$ Monte Carlo samples.
A simple example is an uncorrelated Gaussian noise model, where the noise at a specific time, $\noiset$, is distributed as $\noiset \sim \mathcal{N}(0,\sigma_n)$ with $\sigma_n^2$ being the variance of the detector noise. 
This yields a Gaussian likelihood, $p(\D|\eparam) = \mathcal{N} ( \D-\boldsymbol{s}(\eparam), \sigma_n)$, where $\boldsymbol{s}(\eparam)$ is some signal prediction from the model.
Numerically, we can draw a noise realization from this distribution by taking a signal prediction $\boldsymbol{s}(\eparam)$ and adding random Gaussian noise to it. 
This would give the following dataset $\Dct =  s_{t}(\eparam) + \noiset$, where $t$ ranges across the length of the duration of the signal.
This resulting data set is distributed according the likelihood function, conditioned on a true signal model and parameters $\eparam$.

Extending this further, we can write the hierarchical, population equivalent of this parameter $p(\trig | \hyp)$ for a population model parameterized by $\hyp$.
To evaluate this, we need to expand to all datasets $\D$ and all parameter sets $\eparam$, and marginalize over both these quantities.
\begin{align}\label{eq:alpha}\nonumber
p(\trig | \hyp) \equiv \alpha &= \int d \D \int d\eparam p(\trig, \eparam,\D| \hyp) \,,\\\nonumber
&= \int d \D \int d\eparam p(\trig| \eparam,\D, \hyp) p( \eparam,\D| \hyp)\,,\\
&= \int d \D \int d\eparam p(\trig| \D)p( \D | \eparam) p( \eparam| \hyp)\,,
\end{align}
where we have started by introducing nuisance parameters and marginalizing over them. 
We also used the product rule of probabilities, and noted that (a) once a set of data is specified, the probability of a trigger only depends on that data and (b) once a set of parameters $\eparam$ is specified, the probability of $\D$ is only dependent on parameters $\eparam$ (and not the population model).
We also refer to this quantity as $\alpha$ to conform to past literature and increase readability.
This quantity is the detection efficiency and provides a measure for how ``efficient'' a population model is at producing detectable sources.

We note that for computational purposes, this can be written as 
\begin{equation}
\alpha = \int d\eparam p(\trig| \eparam) p(\eparam | \hyp) \,,
\end{equation}
which allows us to perform this integral by Monte Carlo integration
\begin{subequations}\label{eq:MCefficiency}
\begin{equation}
\alpha \approx \frac{1}{S} \sum_c^S p(\trig| \eparamc)  \,,
\end{equation}
\begin{equation}
\eparamc \sim p(\eparam|\hyp)\,.
\end{equation}
\end{subequations}
We can therefore perform this integral by drawing sources from the underlying population distribution, and averaging over the detection probability for those sources.
If the detection probability function is pre-computed in some form (as we will detail below), this can be reasonably calculated for each population model, generally speaking.

%-------------------------------------------------------------------------------------

%-------------------------------------------------------------------------------------
%\subsubsection{Mixture model with fixed shape}\label{sec:mixingFramework}
%\subsection{Mixture model with fixed shape}\label{sec:mixingFramework}

Building off of the calculations in Appendix~\ref{app:hierarchicalDeriv}, specifically starting with Eq.~\eqref{eq:popPost}, we can tailor this to our particular class of models.
Because we will be using a mixture model, we can fix the subpopulations (fixed distributions of event parameters), but allow the mixing fractions $\{\popfraca\}$ to be variable.
%We will denote these fractions as $\{\popfraca\}$ for $a \in [0,N_{\rm pop})$.
This amounts to using the population likelihood
\begin{equation}
p(\eparam | \{\popfraca \}, \{\hypshapea\})  = \sum_a^{\nclass} \popfraca p(\eparam | \hypshapea)\,,
\end{equation}
for mixing fractions $\popfraca$, individual population distributions $p(\eparam |\hypshapea)$ and $\nclass$ subpopulations.
%Now, $\{\hypshapea\}$ can be thought of as a vector containing shape parameters for each subpopulation (not including the mixing fraction or total number of sources).

In this context, $\{\hypshapea\}$ is fixed, while $\{\popfraca\}$ are free parameters.
Using this population probability, we get the following form for the posterior distribution on the mixing fraction (marginalizing over the total number of sources)
\begin{subequations}
\begin{equation}
p(\{\popfraca\} | \{\DDi\}, \{\trig\},\NOBS,\{\hypshapea\}) \propto \frac{p(\{\popfraca\}| \{\hypshapea\} )\alpha^{-\NOBS}}{p(\{\DDi\}, \{\trig\}, \NOBS)} \prod_{i=0}^{\NOBS}\mathcal{L}_i^{{\rm obs}}\,,
\end{equation}
\begin{equation}
\mathcal{L}_i^{{\rm obs}}  = \int d\eparamdi p(\DDi|\eparamdi)p(\eparamdi|\{\popfraca\}, \{\hypshapea\})\,.
\end{equation}
\end{subequations}
To calculate $\alpha$, we will utilize the form of our mixture model to simplify the calculation.
\begin{align}\nonumber
\alpha &= \int d\D \int d\eparam p(\trig | \D) p(\D | \eparam)p(\eparam|\{\popfraca\}, \{\hypshapea\})\,,\\\nonumber
 &= \sum_a^{\nclass}\popfraca\int d\D \int d\eparam p(\trig | \D) p(\D | \eparam)p(\eparam|\hypshapea)\,,\\
 &= \sum_a^{\nclass}\popfraca \alpha_a\,,
\end{align}
This means we can calculate $\alpha$ for each subpopulation separately, then sum them (weighted) to get the total efficiency of the entire population.
We can utilize a similar trick for the marginalized likelihood, 
\begin{align}\nonumber
\mathcal{L}_i^{{\rm obs}}  &= \int d\eparam p(\DDi|\eparamdi)p(\eparamdi|\{\popfraca\}, \{\hypshapea\})\,,\\ \nonumber
  &= \sum_a^{\nclass}\popfraca \int d\eparamdi p(\DDi|\eparamdi)p(\eparamdi|\hypshapea)\,,\\\nonumber
  &= \sum_a^{\nclass}\popfraca \int d\eparamdi p(\DDi|\eparamdi)p(\eparamdi|\hyp, \classa)\,,\\
  &= \sum_a^{\nclass}\popfraca p(\DDi|\hyp, \classa)\,,
\end{align}
where we make a connection to the original, single event analysis by identifying the integral as the likelihood of a set of data assuming a subpopulation, $\classa$.
With the definitions outlined above, conditioning the individual event likelihood on $\hypshapea$ is equivalent to conditioning jointly on $\hyp$ and $\classa$.
To reuse the results of the single-event analysis, we can rewrite the likelihood as the posterior divided by the prior, giving 
\begin{equation}
\mathcal{L}_i^{{\rm obs}}  = \sum_a^{\nclass}\popfraca \frac{p( \classa | \DDi , \hyp )}{\pi(\classa | \hyp)}\,,
\end{equation}
where we have used similar notation as above, noting the prior for the original analysis using $\pi(\classa | \hyp)$ to differentiate it from the updated, population-informed prior distribution on class $p(\classa|\hyp)$.
This all combines to give the final form of the posterior
\begin{subequations}\label{eq:mixingFractionPost}
\begin{align}\nonumber
p(\{\popfraca\} | \{\DDi\}, \{\trig\}, & \NOBS,\{\hypshapea\}) \propto \frac{ p(\{\popfraca\}|\{\hypshapea\}) (\alpha)^{-\NOBS} }{p(\{\DDi\}, \{\trig\}, \NOBS) } \\
&\times \prod_{i=0}^{\NOBS}\mathcal{L}_i^{{\rm obs}}\,,
\end{align}
\begin{equation}
\mathcal{L}_i^{{\rm obs}}  = \sum_a^{\nclass}\popfraca \frac{p( \classa | \DDi , \hyp )}{\pi(\classa | \hyp)}\,,
\end{equation}
\begin{equation}
\alpha = \sum_a^{\nclass}\popfraca\alpha_a\,,
\end{equation}
\begin{equation}
\alpha_a  = \int d\D \int d\eparam p(\trig | \D) p(\D | \eparam)p(\eparam|\hypshapea)\,,
\end{equation}
\end{subequations}

With Eq.~\eqref{eq:finalPosteriorclass}, Eq.~\eqref{eq:popPost} and Eq.~\eqref{eq:mixingFractionPost}, we have the machinery in hand to understand individual events in the context of their populations and extract meaningful hierarchical information from noisy, biased surveys robustly.
With enough prior information available to ensure no systematic biases, our restricted hierarchical methodology focused on the relative abundances offers a very computational manageable way of understanding populations without extensive simulation.

%To actually perform the inference, we will need a prior on the mixing fractions. 
%We will utilize a broad Dirichlet prior informed by the original simulation, as the mixing fraction is subject to the additional constraint that they must sum to one.
%This all combines to give the final form of the posterior
%\begin{empheq}[box=\fbox]{align}\label{eq:mixingFractionPost}
%p(\hyp | \{d_i\}, \{\trig\},\NOBS) &= \frac{{\rm Dirichlet}(\boldsymbol{f}) (\alpha)^{-\NOBS} }{p(\{d_i\}, \{\trig\}, \NOBS)\NOBS! } \prod_{i=0}^{\NOBS}\mathcal{L}_i^{{\rm obs}}\,,\\
%\mathcal{L}_i^{{\rm obs}}  &= \sum_k^{N_{\rm pop}}f_k \frac{p( \classk | d_i , \hypshapek )}{\pi(\classk | \hypshapek)}\,,\\ 
%\alpha &= \sum_i^{N_{\rm pop}}f_i\alpha_i\,,\\
%\alpha_i  &= \int dd \int d\theta p(\trig | d) p(d | \theta)p(\theta|\hypshapei)\,,
%\end{empheq}
\end{comment}


%%%%%%%%% Old text %%%%%%%%%%%%
%In order to verify the formalism proposed in this work, it is imperative to develop a rigorous testbed for verification and validation.
%Furthermore, the ability to simulate different survey designs in different universes will lead to a much deeper understanding of attainable science goals for the purpose of constructing future surveys.
%To do this, we will consistently simulate the entire pipeline, from the population model with accompanying realizations to characterization of the detection efficiency curves, as a function of survey parameters and population models.
%This simulated data will then be analyzed with the fully robust methods currently employed to infer the model parameters of individual events, consistent with the modeling used to construct the synthetic data.
%Finally, the ensemble of synthetic observations with their accompanying posteriors will be used to infer the underlying population model used to produce said data.
%This fully consistent testbed will enable the calibration and testing of this methodology in an environment free of systematic bias, allowing for proper evaluation of its efficacy.
%Furthermore, extending this testbed to a study on systematic effects related to analyzing data with biased knowledge about detection efficiencies and/or population models can yield much better understanding about the conclusions drawn from current and future hierarchical studies (which is an extension the authors leave to future work).

%We will repeat this analysis for five different population models to adequately evaluate the efficacy of our methodology, denoted by $\{\hyp_0,\hyp_1,\hyp_2,\hyp_3,\hyp_4\}$.
%In an effort to relate to ongoing research and to keep the scope manageable, we will focus on features of the BH mass spectrum being reported by the LVC collaboration~\citep{LIGOScientific:2020kqk,LIGOScientific:2021psn} and whether that feature could be consistent with a subpopulation of PBHs as a specific, well defined test problem. 
%In particular, we will attempt to determine our ability to rule out or confirm the existence of this possible PBH subpopulation given data sets from different universes, with different numbers of PBHs actually contained in the data.
%As a byproduct of studying this particular problem, we will evaluate the ability of this method to contribute to active research surrounding astrophysical populations, such as the population of SOBHs and stellar objects in our galaxy.

%Below, we outline the population models implemented in this work in Sec.~\ref{sec:pop_model}.
%From the population models, we go on to discuss the survey design and selection criteria in Sec.~\ref{sec:det_efficiencies}.
%Next, we move on to outline how we have generated a specific realization of this population model and how we analyzed each synthetic light curve in Sec.~\ref{sec:pop_realization}.
%Finally, we close by discussing the exact prior information we incorporate into our analysis, as well as the details in how we forward model various population models and evaluate the likelihood in Sec.~\ref{sec:forward_modeling}.

%%%%%%%%% OLD TEXT %%%%%%%%%%%%%%%%%%%%
%%To create an actual realization from one of the population models defined above, we begin by randomly drawing event model parameters from the distributions specified by said model.
%A lightcurve is then calculated for the new event, and random noise consistent with our event %likelihood is added to the signal ($n \sim \mathcal{N}(\mu=0,\sigma=0.1)$).
%With a realistic lightcurve consistent with our population model and our likelihood (noise model), we %pass each event through our detection pipeline. 
%If the signal passed the criteria of Table~\ref{tab:selectionCriteria}, it is added to the catalog. 
%We continued this process until we had $\alpha_a N_a$ events for each subpopulation $a \in \{\popA,\popB, \popC\}$.

%Once the ensemble of detections has been constructed, we need the posterior distributions for the %event model parameters for every single event.
%These event model parameters, which fully specify the lightcurve model, include $\{\log F_{\rm Base}, %b_{\rm sff}, \log t_0, \log t_E, \log u_0, \phi, \log \pi_E\}$.
%We sample on the logarithm of certain parameters to compactify the parameter space, easing numerical %instabilities in our sampling algorithm and increasing efficiency. 
%We incorporate the relevant Jacobian factors to properly transform to the specified priors, discussed %below.

%To do this, we explored the parameter space using Markov chain Monte Carlo (MCMC) sampling techniques.
%To execute the sampling itself, we utilized custom MCMC software used in past %research~\citep{Perkins:2021mhb,Perkins:2022fhr}, which has been validated in high dimensional %parameter spaces ($15+$ dimensions) with jagged, multi-modal features in the posterior.
%The software library is built on the concept of parallel %tempering~\citep{PhysRevLett.57.2607,B509983H} to efficiently explore multi-modal posteriors, and %utilizes Fisher information matrices to construct efficient proposal densities. 
%Furthermore, the library implements a version of differential evolution to explore the space in a %generic, model agnostic fashion~\citep{2006S&C....16..239T}, which is a useful supplement to more %targeted proposals. 
%Finally, we seed the sampler with random points from the prior to ensure we are not biased by starting %at the known true values.
%The sampler is allowed to run as long as needed until roughly 1000 independent samples are collected %(as determined by the auto-correlation length).

%For our prior distributions, we used priors we deemed to be appropriately uninformative for each parameter.
%This meant sampling uniformly in the flux $F_{\rm Base}$, the time of maximum magnification $t_0$, the impact parameter $u_0$, the blending fraction $b_{\rm sff}$, and angle $\phi$.
%We sampled uniformly in the \emph{logarithm} of $t_E$ and $\pi_E$ (i.e. uniform in \emph{scale} for these parameters) to ensure proper exploration across the entire parameter space.
%The priors are summarized in Table~\ref{tab:priors}.

%The likelihood distribution $\mathcal{L}(\D|\eparam)$ is consistent with our noise model, a normal distribution with zero mean and $0.1$ variance.
%This is given mathematically as 
%\begin{equation}
%\ln \mathcal{L}(\D|\eparam) \propto -\frac{1}{2} \sum_t^{L_{\rm data}} \frac{(\Dt- I(\eparam,t) )^2 %}{ \sigma_n^2}\,,
%\end{equation}
%where the index $t$ runs across the entire data stream $L_{\rm data}$ and $I(\eparam, t)$ is the prediction for the magnitude from our microlensing model, as a function of the event parameters and time.
%The noise standard deviation, $\sigma_n$, is identical to what was used to generate the data\footnote{This ensures no systematic bias for this preliminary study. Of course, future work could begin to relax this requirement to study systematics or more complicated noise models expected in actual data \citep{Golovich:2020acu}}.

%As illustration, we show the raw data, the true signal, the reconstruction, and residual from our analysis in Fig.~\ref{fig:lightcurveReconstruction} for one specific event in our synthetic catalog.
%This data was created from an event with a long Einstein crossing time ($t_E = 173$ days) and small microlensing parallax ($\pi_E = 0.08$)
%This data was created from an event with a long Einstein crossing time ($t_E = 125$ days) and large microlensing parallax ($\pi_E = 0.35$)

%For reference, the total catalog of detected events in $t_E$-$\pi_E$ space for population models $\Lambda_0$ and $\Lambda_{4}$ are shown in Fig.~\ref{fig:tEPiEDistributionErrorBars0}.
%The points are the $50$-th quantile of the posterior, as calculated by our analysis above, and events from the SOBH and PBH subpopulations show the $1\sigma$ error bars (also calculated from the posteriors).


%%%%%%%%%%%%%%% OLD TEXT BELOW %%%%%%%%%%%%%%%%%%%%%%%

%With the synthetic data created and analyzed, we will now need to prepare our hierarchical framework.
%We will use the formalism derived in Sec~\ref{sec:populations}, specifically Eq.~\eqref{eq:popPost} and Eq.~\eqref{eq:mixingFractionPost}.
%To perform the sampling, we will utilize the same MCMC software as the single event analyses, outlined above.

%When performing the full hyper parameter inference (Appendix~\ref{app:hierarchicalDeriv}), our population models will be constructed from the same distribution families as the injection (two powerlaw distributions and a normal %distribution).
%Furthermore, we will perform inference on the various sets of data with two separate population models: once using all three distributions (producing an unbiased estimate free of systematics) and once using only the two %``expected'' populations: the stellar and SOBH populations only (using only two powerlaws and neglecting the normal distribution).
%The last set of data produced by $\hyp_4$ is the only set of data that can be accurately modeled by both classes, as no PBH lenses actually exist in the data.
%The second class of models will sometimes introduce systematics, providing a good comparison to help gauge our ability to detect the mystery population.
%Both of these classes of models will be used for all five datasets.
%Therefore, our parameter vector will be $\hyp = \{b_\popA,\loc_\popA,\scale_\popA, N_\popA,$ $b_\popB,\loc_\popB,\scale_\popB, N_\popB\}$ and $\hyp = \{b_\popA,\loc_\popA,\scale_\popA, N_\popA,$ $b_\popB,\loc_\popB,\scale_\popB, %N_\popB,$ $\loc_\popC,\scale_\popC, N_\popC\}$ for each class of model, respectively.

%\subsubsection{Prior Probabilities}\label{sec:priorProbs}
%Generally, the priors were chosen to be uninformative.
%The priors for each parameter will be uniform, with the boundaries for parameters associated with stellar and SOBH subpopulations fixed to values commensurate with the uncertainty in the prior understanding of the subpopulation.
%Additionally, the powerlaw populations (the stellar and SOBH populations) will have additional criteria placed on the minimum mass of the distribution (a constraint on the sum of $\loc + \scale$).
%For the SOBH population, we stipulate that the minimum mass of the powerlaw distribution must be in the range of $[2,6]M_{\odot}$, as there is observational evidence for this upper limit from GW observations and x-ray %binaries~\citep{KAGRA:2021duu,Mapelli:2018uds,2010ApJ...725.1918O,2019Sci...366..637T}.
%For the population of most interest to this study (the mysterious PBH population), we also use uniform priors with wide boundaries.
%All of this information is shown in Table~\ref{tab:priorBounds}.

%The priors for each parameter will be uniform, with the boundaries for parameters associated with populations A and B fixed to be $\pm 90\%$ of the injected values.
%\sep{Update.}
%Mathematically, that is 
%\begin{equation}
%p(\hyp_i )\propto 
%\begin{cases}
%&1 \,, \hat{\hyp}_i - |0.9\hat{\hyp}_i| < \hyp_i<\hat{\hyp}_i + |0.9\hat{\hyp}_i|\,,\\
%&0 \,, {\rm otherwise}\,,
%\end{cases}
%\end{equation}
%for parameters $\hyp_i \in \{b_A, \loc_A, \scale_A, N_A,b_B, \loc_B, \scale_B, N_B \}$, where $\hat{\hyp}_i$ is the true, injected parameter for the population model generating the data.
%The added stipulation for $\loc_{A,B}$ and $\scale_{A,B}$ (which control the minimum mass of these two populations through the combination $m_{{\rm min},(A,B)} = \loc_{A,B} + \scale_{A,B}$) is that the sum must be greater than $0.01$.
%In other words, $m_{{\rm min}, (A,B)} > 0.01$.
%These prior boundaries are meant to reflect a reasonable (but not infinite) amount of uncertainty on the populations that we know something about, in principle.
%For population C (which is meant to represent an open question in physics and could potentially come from exotic origins), we use a much wider prior given by 
%\begin{align}
%p(\loc_C )&\propto 
%\begin{cases}
%&1 \,, 2 < \loc_C<80\,,\\
%&0 \,, {\rm otherwise}\,,
%\end{cases}\\
%p(\scale_C )&\propto 
%\begin{cases}
%&1 \,, 1 < \scale_C<10\,,\\
%&0 \,, {\rm otherwise}\,,
%\end{cases}\\
%p(N_C )&\propto 
%\begin{cases}
%&1 \,, 0 < N_C<16,457\,,\\
%&0 \,, {\rm otherwise}\,,
%\end{cases}
%\end{align}
%where the upper limit of $N_C$ is the total number of sources (detected and not) in the original data.

%To visualize the credible region for the mass distribution given distributions on the hyper-parameters, we simply calculate the mass distribution marginalized over population models.
%This is the posterior predictive distribution~\cite{}, given by
%\begin{equation}
%p(M) = \int d\hyp p(M|\hyp) p(\hyp|\{d\},\{\trig\}, \NOBS)\,,
%\end{equation}
%where $p(\hyp|\{d\}, \{\trig\}, \NOBS)$ is the posterior distribution.
%In practice, we can again evaluate this type of integral with Monte Carlo integration.
%We first divide the mass range into a grid, $M_i$, integrating at each point in mass space.
%Then, at each $M_i$, we use our posterior distribution samples to calculate the $90\%$ confidence region.
%In practice, this can simply be done by calculating the mass distribution for a variety of posterior samples, then using standard algorithms from, e.g. \software{NumPy}, to calculate the $90$-th quantile along the mass axis.
%We can do this same process with the prior (called the prior predictive distribution) by replacing the posterior above with the prior distribution.
%This process gives the mass PDF of each population shown in Fig.~\ref{fig:priorReconstruction}.

%\begin{figure}
%\includegraphics[width=\linewidth]{ci_log10mass_pdfPrior.pdf}
%\caption{
%	The reconstruction of the mass PDF for each population, as calculated from random draws from the prior space. 
%	The lines each represent the true, injected mass PDF for each individual population.
%	The shaded region is the $90\%$ credible region.
%}\label{fig:priorReconstruction}
%\end{figure}
%
%\begin{figure}
%\includegraphics[width=\linewidth]{ci_log10mass_pdf_total_reconstructionPrior.pdf}
%\caption{
%	The reconstruction of the mass PDF for the total population (the weighted sum of each subpopulation), as calculated from random draws from the prior space when considering a fully flexible model. 
%	The red shading indicates the $90\%$ confidence reconstruction of the mass distribution from the prior distribution, while the gray line indicates the true distribution, and the gray histogram represents the observed data generated from the distribution.
%	Note, the histogram reflects observation bias while the gray curve reflects the true, intrinsic distribution.
%}\label{fig:priorReconstruction}
%\end{figure}



%\begin{figure}
%\includegraphics[width=\linewidth]{mixing_frac_corner_full_bayesianPrior.pdf}
%\caption{
%	The relative abundances of the different populations, as calculated from samples drawn from the prior when considering the entire population model.
%	The blue lines represent the values of the true model.
%}\label{fig:priorMixingFractions}
%\end{figure}

%When we focus on the relative abundances only and use fixed distributions for $t_E$-$\pi_E$ space for each subpopulation (the restricted analysis in Sec.~\ref{sec:populations}), we will use the parameter vector $\{\fracA, \fracB %,\fracC\}$.
%As the additional constraint that $\sum_a \popfraca=1$ removes an independent parameter, we will only sample on $\fracA$ and $\fracB$.
%To actually perform the inference, we will need a prior on the relative abundances. 
%Following~\cite{Golovich:2020acu}, we will utilize a broad Dirichlet prior informed by the original simulation, as the relative abundances are subject to the additional constraint that they must sum to one.
%The Dirichlet distribution is parametrized by a vector $\boldsymbol{a}$, which we specify as 
%\begin{equation}
%\boldsymbol{a} =  (\hat{\popfrac}-{\rm min}(\hat{\popfrac}))  + c\,,
%\end{equation}
%where $c$ controls the width of the prior, and $\hat{\popfrac}$ is a vector of the relative abundances of the injected population model.
%We have chosen $c=1$ to produce a broad, uninformative prior on the parameters.
%We chose this prior because it naturally satisfies the requirement that the relative abundances sum to 1, and the specified vector $\boldsymbol{a}$ yields a largely uninformative prior.
%These priors are shown in Fig.~\ref{fig:priorMixingFractionsFixedShape} for the mixing ratios themselves and the prior space on the lens mass PDF is shown in Fig.~\ref{fig:priorReconstructionFixedModel} .
%This all combines to give the final form of the posterior
%\begin{empheq}[box=\fbox]{align}\label{eq:mixingFractionPostFinal}
%p(\hyp | \{d_i\}, \{\trig\},\NOBS) &= \frac{{\rm Dirichlet}(\boldsymbol{f}) (\alpha)^{-\NOBS} }{p(\{d_i\}, \{\trig\}, \NOBS)\NOBS! } \prod_{i=0}^{\NOBS}\mathcal{L}_i^{{\rm obs}}\,,\\
%\mathcal{L}_i^{{\rm obs}}  &= \sum_k^{N_{\rm pop}}f_k \frac{p( \classk | d_i , \hypshapek )}{\pi(\classk | \hypshapek)}\,,\\ 
%\alpha &= \sum_i^{N_{\rm pop}}f_i\alpha_i\,,\\
%\alpha_i  &= \int dd \int d\theta p(\trig | d) p(d | \theta)p(\theta|\hypshapei)\,,
%\end{empheq}

%\begin{figure}
%\includegraphics[width=\linewidth]{fraction_recoveryPrior.pdf}
%\caption{
%	The relative abundances of the different populations, as calculated from samples drawn from the prior when considering inference only on the relative abundances.
%	The prior is a Dirichlet prior, with parameters of that distribution discussed in the text.
%	The blue lines represent the values of the true model.
%}\label{fig:priorMixingFractionsFixedShape}
%\end{figure}
%
%\begin{figure}
%\includegraphics[width=\linewidth]{ci_log10mass_pdf_total_reconstruction_fixedModelPrior.pdf}
%\caption{
%	The reconstruction of the mass PDF for the total population (the weighted sum of each subpopulation), as calculated from random draws from the prior space when considering a fixed model and only inferring the relative abundances. 
%	The red shading indicates the $90\%$ confidence reconstruction of the mass distribution from the prior distribution, while the gray line indicates the true distribution, and the gray histogram represents the observed data generated from the distribution.
%	Note, the histogram reflects observation bias while the gray curve reflects the true, intrinsic distribution.
%	\sep{Added this figure and some text about it.}
%}\label{fig:priorReconstructionFixedModel}
%\end{figure}

\begin{comment}

\subsubsection{Population Forward Modeling and Population Likelihood Evaluation }

\sepc{Remove section?}

When inferring the full population model and not just the relative abundances, we need to produce many population simulations to perform robust inference.
From Eq.~\eqref{eq:popPost}, we see that we need a prediction for $t_E$-$\pi_E$ distributions of the lensing events from the population model currently being evaluated.
The maximally robust method of performing this calculation is to re-perform the simulation at each likelihood evaluation.
As our toy model is analytic in the mass distribution, we can simply redraw all the requisite parameters to produce a representative sampling ($10^5$ sources per population per likelihood evaluation) and estimate the distributions through this Monte Carlo simulation. 
This yields the most accurate results, and we therefore use this as a baseline to test our analysis framework.

However, this method is computationally intractable when working with real data.
When considering realistic populations, re-drawing a population realization would require performing a full simulation, al\'a PopSyCLE.
To illustrate a simple method to potentially reduce the computational cost when using real data, we will also run our analysis by taking a large "reference" simulation performed at very high resolution and importance sampling from that distribution to obtain derivative simulations.
To do this, we will simply use weights given by
\begin{equation}\label{eq:weights}
w_i = \frac{p_{\rm target}(M) }{p_{\rm ref}(M)}\,,
\end{equation}
for the $i$-th sample, where $p_{\rm target}(M)$ is the target mass distribution currently being evaluated, and $p_{\rm ref}(M)$ is the mass distribution used to synthesize the reference simulation.
If we were investigating event model parameters beyond the mass, we would extend these probability density functions to their joint distributions.
To provide accurate results using this method, the reference simulation must be broad enough to adequately cover the entire parameter space.
To ensure this, our reference simulation was produced with the following mass distributions for the three subpopulations are shown in Table.~\ref{tab:referencePopulationParameters}

\begin{table}
\centering
\begin{tabularx}{0.8\linewidth} { 
   >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X 
}
\hline\hline 
Population & Distribution ($p(M)$) & Parameters \\\hline \hline
$\popA$ & Powerlaw & \makecell{$b_\popA=2$ \\$\loc_\popA = -0.99$\\$\scale_\popA = 1$} \\\hline
$\popB$ & Powerlaw & \makecell{$b_\popB=0.5$ \\$\loc_\popB = -5.99$\\$\scale_\popB = 6$} \\\hline
$\popC$ & Normal & \makecell{$\loc_\popC = 30$\\$\scale_\popC = 100$} \\
\hline\hline 
\end{tabularx}
\caption{
	Above are shown the mass distributions for each subpopulation of lenses used to generate the reference simulation.
	The distributions and the parameters are defined in Eq.~\eqref{eq:pareto} and Eq.~\eqref{eq:normal}.
}\label{tab:referencePopulationParameters}
\end{table}

To calculate the actual likelihood, we now need two things: (1) an approximation of the distribution in $t_E$-$\pi_E$ space for the target population model and (2) the population efficiency, $\alpha$.
To calculate the $t_E$-$\pi_E$ distribution, we simply histogram the samples from our simulation in a $30 \times 30$ grid in $\log_{10} t_E$ and $\log_{10} \pi_E$ using \software{BOOST}~\cite{}.
To calculate the population detection efficiency, we perform the Monte Carlo integral of Eq.~\eqref{eq:MCefficiency} using the population simulation.
For both of these calculations, the weights of Eq.~\eqref{eq:weights} are used when importance sampling to correct for differences in the distributions.

\begin{figure}
\includegraphics[width=\linewidth]{referencePDFs.pdf}
\caption{
	\sepc{Change labels.}
	The analytic mass PDFs for each subpopulation used in the reference simulation when importance sampling.
	The distributions were chosen to provide high fidelity in regions of mass parameter space with large impact in the calculation while still adequately covering the entire space.
}\label{fig:referencePDFs}
\end{figure}

When we perform the analysis with a fixed-shape population model and only infer the relative abundances, we use the shape parameters from the true distribution used to generate the data (i.e. $\{b_\popA, \loc_\popA, \scale_\popA,b_\popB, \loc_\popB, \scale_\popB, \loc_\popC, \scale_\popC\}$ from the population model used to generate the data).
This removes any systematic bias from the analysis, giving a best-case scenario to benchmark this framework.
Future work could investigate the effects of various systematic effects by inferring the mass model from the data using a slightly incorrect population model, but we leave that for future investigations.

\end{comment}

%For the hierarchical inference used in this work, we have two different versions: the general framework used to infer the different distributions of the subpopulations and the simplified restricted analysis assuming a mixture model and only inferring the relative abundances.
%Both of these frameworks are detailed in Sec.~\ref{sec:populations}.
%We will discuss the results of these two analysis in Sec.~\ref{sec:generalPopResults} and Sec.~\ref{sec:mixingFractionInference}, respectively.


%\subsection{Full Model Inference}\label{sec:generalPopResults}

%We begin by first asking the simple question: how many lenses in the data are likely to belong to each category of object (i.e., star, SOBH or PBH)? 
%We know that classifying a single event from photometric data alone is difficult (see Sec.~\ref{sec:source_classification}), but does that mean we have no chance of inferring the relative abundance of each category? 
%We first focus on the relative abundance of the PBH subpopulation (the main science question we focus on in this study) shown in Fig.~\ref{fig:fractionRidge}.
%The distributions are separated by the datasets $\hyp_i$.
%From this figure, we see that our ability to detect PBHs as a subset of lensing objects in the catalog varies.
%When a significant number of PBHs truly exist in the data (our baseline test, $\hyp_0$), we find strong evidence for the existence of this subpopulation (indicated by the PBH relative abundance posterior being inconsistent with zero).
%As the number of PBHs in the datasets begins to shrink, our ability to distinguish between the existence or non-existence of this subpopulation also diminishes.
%Dataset $\hyp_1$ also shows a substantial preference for including the PBH subpopulation in the modeling, again disfavoring $\fracC$ being zero, while dataset $\hyp_2$ shows a mild preference for the %existence of the PBH subpopulation.
%Conversely, datasets $\hyp_3$ and $\hyp_4$ are consistent with the PBH population not existing.
%Even in the case of $\hyp_3$ and $\hyp_4$, we can still place a robust bound on the upper limit of this subpopulations contribution (both to DM and to the lensing population as a whole), plateauing around $20$-$25\%$ of the DM fraction ($f_{\popC}$) and about $1\%$ of all lensing objects in the lensing population ($\fracC$).


%Considering the astrophysical subpopulations, we find complementary diagnostics.
%In particular, the mixing fraction of SOBHs encodes some meaningful information about the existence of a third subpopulation of PBHs, shown in Fig.~\ref{fig:fractionRidge}.
%In this figure, the posterior distribution on the mixing fraction of the SOBH population is shown as determined by both classes of models: the two population configuration (hatched) and the three population configuration (non-hatched).
%When a substantial number of PBHs exist in the data ($\hyp_0$) and two populations are used to analyze the data (hatched distribution), the fraction of SOBH lenses is roughly a factor of five larger than the number expected from the initial simulation.
%The SOBH subpopulation is simply absorbing the missing number of PBH lenses into SOBH subpopulation, which is not surprising.
%As the expected number of SOBHs in the Milky Way is uncertain to a factor of $\sim100$~\citep{Samland1998,1996ApJ...457..834T,1992eocm.rept...29V}, this fact alone is not an immediate signature of exotic physics.

%However, the degeneracy has a bi-modality, exhibited in the separation of the two and three population model posteriors (hatched against non-hatched).
%If the two BH populations (SOBH and PBH) were perfectly degenerate, the two distributions would be wide but overlapping, extending from $0$ to $\sim 0.05$ in a continuous distribution for both classes of models (the sum of the two subpopulations PBH and SOBH always accounting for the total contribution of both subpopulations).
%This would indicate that the PBH subpopulation does not contribute to explaining the data in a meaningful way, with the caveat that the total number of predicted BHs agrees with the data.
%However, because the population model favors \emph{not} having a large number of SOBH sources but instead tends toward an SOBH population consistent with zero relative abundance when including a PBH subpopulation in the modeling, a hierarchy emerges in the explaining power of each class of population model.
%In this case, using both powerlaw and Gaussian distributions to describe the BH population is more informative than the population model which neglects the PBH subpopulation.
%As the second mode in the three subpopulation model posterior (having an SOBH subpopulation with $\sim 0.05$ relative abundance) is equally allowed as the two population analysis, but disfavored, the immediate conclusion is that using both a powerlaw and Gaussian distribution for BHs as opposed to just a powerlaw is more informative and describes the data in a more meaningful way.

%We now consider how well these methods can reconstruct the lens mass distribution as a whole.
%These results are shown in Fig.~\ref{fig:massReconRidge}, where we see this method can lead to unbiased inference that improves on the priors used in this study.
%The top panel of the figure shows the full range of mass distributions for the total lensing population allowed by the prior (calculated by randomly sampling from the prior defined in Sec.~\ref{sec:pop_realization}). 
%Each set of data produced from the different injected population models ($\hyp_i$) are shown in the subsequent panels, with the $90\%$ confidence reconstruction of the mass distribution from the posterior distribution of the hierarchical parameters for each class of analysis (assuming two or three subpopulation components) shown alongside the true distribution.
%We can see that in all cases where systematic bias is not present, we infer a distribution in agreement with the true distribution to within $90\%$ credibility.
%The posterior reconstructions are also noticeably different than our prior reconstructions, indicating a substantial amount of information was learned in the inference process.

\begin{comment}
Before discussing the myriad of inference products this type of analysis can potentially produce, we first ask the simple question: can the mass distribution of the lensing population (a quantity not directly measured but only calculable through a lossy mapping of different event parameters to observables) be measured in an unbiased and informative way? 
While ``informative'' is dependent on the exact goals of the study in question, Fig.~\ref{fig:massReconRidge} shows that, indeed, this route of analysis can lead to unbiased inference that improves on the priors used in this study.
The top panel of the figure shows the full range of mass distributions for the total lensing population allowed by the prior (calculated by randomly sampling from the prior defined in Sec.~\ref{sec:priorProbs}). 
Each set of data produced from the different injected population models ($\hyp_i$) are shown in the subsequent panels, with the $90\%$ confidence reconstruction of the mass distribution from the posterior distribution of the hierarchical parameters for each class of analysis (assuming two or three sub population components) shown alongside the true distribution.
We can see that in all cases where systematic bias is not present, we infer a distribution in agreement with the true distribution to within $90\%$ credibility.
We also see the posterior reconstructions are noticeably different than our prior reconstructions, indicating a substantial amount of information was learned in the inference process.
\end{comment}

%The disagreement between the two classes of models (those that assume two or three subpopulations) becomes obvious when the data is truly produced with a significant number of PBH lenses. 
%Without the flexibility of the Gaussian subpopulation component, the SOBH powerlaw population shifts to compensate for the missing category of lenses.This can be seen in the stark differences between the posteriors for the relative abundance of SOBHs shown in Fig.~\ref{fig:fractionRidge}.
%However, there are indicators in the mass spectrum of ``fine-tuning''.
%The two subpopulation model inference favors a very narrow distribution in the SOBH segment of the population, indicating a narrow range of hyperparameter space that yields reasonable %agreement with the data.


%see one model is more ``complex'' because of increased dimensionality (the three subpopulation class of model) while the other requires fine tuning of the hyper parameters to explain the %data (the two subpopulation class of model).

%This is a certain aspect of model complexity that must be considered when evaluating competing models: in the one case, one model is more ``complex'' because of increased dimensionality %(the three subpopulation class of model) while the other requires fine tuning of the hyper parameters to explain the data (the two subpopulation class of model).
%This figure represents an initial diagnostic in the model selection problem of determining the evidence for the additional subpopulation of PBH lenses, where we see a systematic inability %of the simpler model to accurately recover the true distribution.
%Unfortunately, the mass distribution of the lensing population is not the direct observable, but only measured through the intermediary lensing parameters $t_E$ and $\pi_E$.

%Furthermore, the $\hyp_0$ and $\hyp_1$ simulations show information can be gained about the internal structure of this Gaussian sub-population component as well.
%We see strong evidence for the bump around the correct location of $30 M_{\odot}$ (more clearly shown by the posterior distribution for the $\loc_{\popC}$ parameter in Fig.~\ref{fig:PBHLocationRidge}).
%The reconstruction is somewhat wider than the injected Gaussian component, but this is simply a reflection that our analysis is not as sensitive to the width of this mystery mass distribution.
%The posterior on the width of the Gaussian component $\scale_{\popC}$ is marginally different than the prior distribution, and the prior distribution puts more weight on wider distributions than what was used to create the data.
%In the case of $\hyp_2$ to $\hyp_4$, the only conclusion from this analysis is that the data did not favor a high mass component to the lensing population, placing an upper bound on the mass range of this subpopulation.
%As the lower mass part of the spectrum overlaps largely with the stellar population (vastly dominating the catalog by numbers), the extra flexibility can be absorbed into the noise of the primary population.

\begin{comment}
Ultimately, the relative abundance of each population represents the leading order science we aim to address. 
We plot the relevant posteriors for the abundance of the PBH subpopulation in Fig.~\ref{fig:fractionRidge}, separated by the datasets $\hyp_i$.
From this figure, we see that our ability to detect PBHs as a subset of lensing objects in the catalog varies.
When a significant number of PBHs truly exist in the data (our baseline test, $\hyp_0$), we find strong evidence for the existing of this subpopulation.
Our posterior for the relative abundance is inconsistent with zero, indicating that PBHs contribute meaningfully to explaining the data.
As the number of PBHs in the datasets begins to shrink, our ability to distinguish between the existence or non-existence of this subpopulation also diminishes.
Dataset $\hyp_1$ still shows a substantial preference for including the PBH subpopulation in the modeling, again disfavoring $\fracC$ being zero.
Conversely, $\hyp_2$ through $\hyp_4$ are consistent with the PBH population not existing.
In this case, however, we can place a robust bound on the upper limit of this subpopulations contribution (both to DM and to the lensing population as a whole), plateauing around $20$-$25\%$ of the DM fraction ($f_{\popC}$) and about $1\%$ of all lensing objects in the lensing population ($\fracC$).

\begin{figure*}
\includegraphics[width=.48\linewidth]{PBHPopFractionRidge.pdf}
\includegraphics[width=.48\linewidth]{SOBHPopFractionRidge.pdf}
\caption{
	Shown above are the Posterior distributions for the mixing fraction or relative abundance of the PBH (left) and SOBH (right) subpopulation and its contribution to the total DM mass ($\fracC$ and $f_{\rm PBH}$ on the left and $\fracB$ on the right).
	Vertical lines indicate the true value used to create the data.
	The prior on the absolute abundance of each subpopulation, $N_{\classa}$, was uniform between $1$ and twice the number of lenses in the specific simulation, which translated to a prior on the relative abundance that was broad (between $0$ and $1$), but mildly peaked around $0.5$.
	For the PBH subpopulation, we can see that we have an indication that the PBH subpopulation contributes meaningfully to the explanation of the data, due to the posteriors being inconsistent with zero in the case of datasets $\hyp_0$ and $\hyp_1$. 
	In the case of the other datasets ($\hyp_2$ to $\hyp_4$), we can merely make statements about the maximum contribution of PBHs to the lensing population ($\sim1\%$) and their contribution to the DM fraction ($\sim 20-25\%$).
	For the SOBH subpopulation, we see a separation of the posteriors when using two and three subpopulations.
	This is an indicator that the Gaussian component leads to a better description of the data, indicating a need for the more complex model.
}\label{fig:fractionRidge}
\end{figure*}

\end{comment}

\begin{comment}
Moving on to consider the astrophysical subpopulations, we find complementary diagnostics in the problem of detecting PBHs in the parameters controlling the SOBH distributions.
Of particular note, the mixing fraction of SOBHs also encodes some meaningful information about this question of the existence of a third subpopulation, shown in Fig.~\ref{fig:fractionRidge}.
We see in this figure the posterior distribution on the mixing fraction of the SOBH population as determined by both classes of models: the two population configuration (hatched) and the three population configuration (non-hatched).
The first observation to be made from this figure is that when a substantial number of PBHs exist in the data ($\hyp_0$) and two populations are used to analyze the data (hatched distribution), the fraction of SOBH lenses is roughly fives the number expected from the initial simulation.
The SOBH subpopulation is simply absorbing the missing number of PBH lenses into SOBH lenses, which is not surprising.
As the expected number of SOBHs in the Milky Way is uncertain to a factor of $\sim100$~\citep{Samland1998,1996ApJ...457..834T,1992eocm.rept...29V}, this fact alone is not an immediate signature of exotic physics.
However, the degeneracy has a bi-modality, exhibited in the separation of the two and three population model posteriors (hatched against non-hatched).
If the two populations (SOBH and PBH) were perfectly degenerate, the two distributions would be wide but overlapping, extending from $0$ to $\sim 0.05$ in a continuous distribution for both classes of models (the sum of the two subpopulations PBH and SOBH always accounting for the total contribution of both subpopulations).
This would indicate that the PBH subpopulation does not contribute to explaining the data in a meaningful way, with the caveat that the total number of predicted BHs agrees with the data.
However, the fact that when three populations are used, the model favors \emph{not} having a large number of SOBH sources, but instead tends toward an SOBH population consistent with zero relative abundance, indicates a hierarchy in the explaining power of each class of model.
As the second mode in the three subpopulation model posterior (having an SOBH subpopulation with $\sim 0.05$ relative abundance) is equally allowed as the two population analysis, but disfavored, the immediate conclusion is that using both a powerlaw and Gaussian distribution for BHs as opposed to just a powerlaw is more informative and describes the data in a more meaningful way.
\end{comment}

%\begin{figure}
%\includegraphics[width=\linewidth]{SOBHPopFractionRidge.pdf}
%\caption{
%	Shown above are the posterior distributions on the relative abundance of the SOBH subpopulation ($\fracB$) separated by dataset ($\hyp_i$) and by the model used for inference (two or three population components).
%	In the case of a strong population of PBHs in the data ($\hyp_0$), there is a strong separation of the distributions (also somewhat present in $\hyp_1$, but to a much less degree).
%	The prior on this parameter is not analytic, as the sampled parameter was the number of sources, not the relative abundance.
%	The prior on the relative abundance was uniform between $1$ and twice the number of lenses in the specific simulation, which translated to a prior on the relative abundance that was broad (between $0$ and $1$), but mildly peaked around $0.5$.
%	This separation is a symptom of the drop in explaining power when using two subpopulations as opposed to three.
%	This is an indicator that the Gaussian component leads to a better description of the data, indicating a need for the more complex model.
%}\label{fig:SOBHPopFractionRidge}
%\end{figure}

%\begin{figure}
%\includegraphics[width=\linewidth]{bayesFactorLikelihoodComp.pdf}
%\caption{
%	Shown along the left axis are the logarithm of the Bayes' factor between the two and three subpopulation class of models for each set of data $\hyp_i$.
%	Along the right axis are shown the difference in the logarithm of the maximum likelihood values between the two and three subpopulation class of model for each set of data $\hyp_i$.
%	While the Bayes' factor statistic does not suggest strong evidence for a PBH subpopulation in any dataset, the ability to differentiate between the two models (two or three subpopulations) clearly improves as the number of PBH lenses actually in the data increases (from $\hyp_4$ to $\hyp_0$).
%}\label{fig:bayesFactorLikelihoodComp}
%\end{figure}

%Some of the conclusions based on Fig.~\ref{fig:massReconRidge} and Fig.~\ref{fig:fractionRidge} allude to a breakdown of the model's ability to sufficiently explain the data.
%There are two natural statistics to quantify the consistency between multiple models and the data that we will employ: the Bayes' factor and the maximum likelihood estimate.
%Traditionally, the Bayes' factor is a widely accepted method for Bayesian model selection.
%This direct comparison between two models has many benefits, including its direct interpretation (this ratio is a direct comparison of the posterior probability for each model) and this method %accounts for changes in model complexity.
%However, the Bayes' factor calculation comes with well-known drawbacks as well. 
%Namely, the most common criticism is its sensitivity to the priors. 
%For this reason, the Bayes' factor is not a perfect metric for model comparison, but does provide good insight into the problem.

%\sepc{We can leave this out, if this is information that is obvious. I think it's important to understanding the Bayes' factor results, though.}
%%However, Bayes' factor calculations have nuances that some might characterize as a limitation while others characterize as a feature.
%However, Bayes' factor calculations have nuances that can be viewed as limitations.
%The calculation is nothing more than the direct comparison of the \emph{entire} model, including the form of the likelihood and the prior in addition to the actual \emph{population} model itself, $\hyp$.
%One can arbitrarily tune the Bayes' factor by widening the prior range of one model, even if the posterior is unchanged, as the result of the Occam factor.
%Neglecting to account for this fact or obscuring its impact can lead to biased or misleading results.
%Conversely, truly Bayesian calculations will always be dependent on the choice of priors, of course, and so this fact is unsurprising.
%%Their role in the calculation has exactly equal footing, mathematically, as the likelihood itself.
%The fact that the analysis is sensitive to this choice simply highlights the need for careful consideration of the priors being employed.
%However, this does introduce concerns when meaningful, generally accepted priors can not be found.
%As such, it can be seen as a useful (albeit not all-encompassing) metric for the model selection problem.
%To ascertain the impact of the priors on the Bayes' factor calculation, we can also compare the maximum likelihood values between models.
%Both of these statistical criteria comparing the two and three subpopulation classes of models for each dataset are shown in Fig.~\ref{fig:bayesFactorLikelihoodComp}, with the (logarithmic) difference in maximum likelihood shown along the right axis and the logarithm of the Bayes' factor shown along the left axis.

%In this figure, we can see that both metrics track one another very well, showing that the improvement in Bayes' factor is driven by the improvement to the likelihood.
%In Fig.~\ref{fig:bayesFactorLikelihoodComp}, we show the Bayes' factor calculation for all sets of data.
%The Bayes' factor calculation never produces evidence for a PBH subpopulation.
%This is largely due to the wide, uninformative priors used for this toy problem (Sec.~\ref{sec:verification}).
%The flexibility of the two subpopulation model is enough to allow for fine tuning and to ``absorb'' the PBH populations in each data set into the SOBH population, discussed in detail above.
%This is clear from the posteriors on the mixing fraction for the SOBH population shown in Fig.~\ref{fig:fractionRidge}, where the $\hyp_0$ data set suggests four to five times the number of SOBH lenses than what actually exists in the data.
%We can also see this in Fig.~\ref{fig:massReconRidge}, where the reconstructed mass distribution for the SOBH population in the $\hyp_0$ data set is very narrow and significantly higher than the true distribution, suggesting a small part of the hyperparameter space allows the two subpopulation model to capture the main affects of the third subpopulation without actually needing a third subpopulation.
%While sufficient evidence cannot be found for any of the data sets in isolation (considering only the Bayes' factors), there is a strong trend in this figure showing that as the number of PBH lenses in the data increases, our ability to distinguish between the two population model classes improves significantly.
%The difference in the logarithm of the maximum likelihood increases by about 4-5 (equivalent to the maximum likelihood value of the three subpopulation model increasing by a factor of $\sim100\times$) and the logarithm of the Bayes' factor increases by $\sim 7$.
%While conclusive evidence for a subpopulation of PBH lenses cannot be claimed in this toy example (when only considering the Bayes' factor statistic alone), the absolute scale of the Bayes' factor is less important than the strong trend we see in Fig.~\ref{fig:bayesFactorLikelihoodComp}. 
%Said trend suggests careful application of appropriate, informative priors and future data sets have potential to provide a different conclusion.

%\begin{figure}
%\includegraphics[width=\linewidth]{SOBHMinMassRidge.pdf}
%\caption{
%	Shown above are the posterior distributions for the minimum mass of the SOBH Pareto distribution ($M_{\rm min, \popB}$).
%	The vertical lines indicate the true value used to create each data set, while the hatched distributions refer to inference performed assuming two subpopulations and unhatched distributions were inferred assuming three subpopulations.
%	The prior for this parameter was a uniform distribution between $2 M_{\odot}$ and $6M_{\odot}$.
%	We see that we can not infer the minimum mass of the SOBH Pareto distribution, regardless of the data set or population model employed.
%	The data sets and type of data (photometry only) do not contain enough information to place robust bounds on the minimum mass of the SOBH population that would be useful in measuring things like the NS-BH mass gap~\cite{}. 		
%}\label{fig:SOBHMinMassRidge}
%\end{figure}

%Beyond looking for exotic physics, we can assess our ability to infer certain features of astrophysical subpopulations, such as the minimum mass parameter for the stellar and SOBH subpopulations, $M_{\rm min, \popA}$ and $M_{\rm min, \popB}$, respectively.
%These posterior distributions are shown in Fig.~\ref{fig:MinMassRidge}, separated both by dataset ($\hyp_i$) and the inference model (two or three population components).
%In the case of the minimum mass, our analysis makes two robust conclusions: the stellar minimum mass can be well inferred from our data set, while the SOBH minimum mass is never well inferred.
%In the case of the stellar subpopulation, we see a tight constraint of $0.08 M_{\odot}\pm 0.02 M_{\odot}$, regardless of the population model or data set used.
%As a reminder, the prior for this parameter is between $0.01$ and $1M_{\odot}$.
%The large number of stellar lenses in the data suggests there is enough information (even in the noisy posteriors for the individual events) to make robust claims about the minimum mass, given our simplistic toy problem.
%In contrast, the minimum mass for the SOBH population is never well measured, always approximately just recovering the prior distribution (uniform between $2$ and $6M_{\odot}$.
%The posterior does not provide information that would be helpful in answering questions related to the existence and properties of the mass gap between NSs and %BHs~\citep{2011ApJ...741..103F,2010ApJ...725.1918O,2001ApJ...554..548F}.
%While there is slight variation between the data sets and population models used for inference, the distribution is not informative.
%This difference between conclusions for the stellar subpopulation and SOBH subpopulation most likely comes from the vast difference in the expected number of lenses coming from each subpopulation, with thousands of stellar lenses containing much more data than the tens of SOBH lenses.
%While this conclusion should be reevaluated for future surveys with tighter measurements and larger catalog sizes ~\citep[such as for Roman][]{2015arXiv150303757S} or when other data is taken %into account (such as astrometry), our initial analysis using photometric only, OGLE-type data does not give confidence that this will be a measurable feature, with our models.

%Other parameters of interest for the astrophysical stellar and SOBH subpopulations are the shape parameters, $b_{\popA}$ and $b_{\popB}$.
%The posterior distribution for these two parameters are shown in Fig.~\ref{fig:PowerRidge}.
%In the case of the stellar subpopulation, the posteriors generally match those of the prior (uniform between $0.1$ and $10$).
%This might seem surprising, given the reconstruction of the stellar subpopulation in Fig.~\ref{fig:massReconRidge} seems to be doing well and seems informative.
%However, the broad posteriors for $b_{\popA}$ are principally caused by the correlation with the location parameter, $\loc_{\popA}$, which is a symptom of the flexible model we used (a Pareto type-II distribution).
%This location parameter has the effect of rounding the low mass component of the distribution, resulting in a high degeneracy with the shape parameter $b_{\popA}$.
%This is shown graphically in Fig.~\ref{fig:bmuStarCov}, where the posterior and prior for these two parameters are shown together(from the $\hyp_0$ data set and assuming the two subpopulation model).
%While a certain linear combination of these two parameters is constrained very tightly, the orthogonal combination is almost totally unconstrained (along the contours of the posterior).
%This leads to the wide, marginalized posteriors for $b_{\popA}$ in Fig.~\ref{fig:PowerRidge}, despite significant information being extracted from the data about the shape of this distribution. 


%In the case that one attempts to simultaneously search for exotic physics by including additional flexibility (i.e., including a third subpopulation), the posteriors are largely uninformative. 
%However, when one focuses on astrophysics alone (by only including two subpopulations, in our case), informative posteriors can be derived.
%This potentially introduces systematics, of course, where we see systematic error in the posterior derived from $\hyp_0$.
%However, in the case of no systematics (dataset $\hyp_4$), we see a reasonably tight constraint on the SOBH shape parameter.
%As an interesting note, the posteriors on the SOBH shape parameter constraints are tighter in the case of serious systematics (using two subpopulations to analyze $\hyp_0$ data, for instance).
%This is another symptom of the fine-tuning issue discussed earlier, where the ``wrong'' model can still reasonably explain the data if the hyperparameters take very specific combinations of values.

%\begin{figure}
%\includegraphics[width=\linewidth]{SOBHpowerindexRidge.pdf}
%\caption{
%	The posterior distribution for the shape parameter of the SOBH Pareto distribution ($b_{\popB}$), separated by population model (models with two subpopulation represented with hatched distributions) and by set of data $\hyp_i$.
%	The vertical lines indicate the true value used to create the data.
%	The prior for this parameter was uniform between $0.1$ and $10$.
%	In the case of assuming three subpopulations, the posteriors are uninformative.
%	However, when only considering two subpopulations (thereby focusing on the astrophysics as opposed to exotic physics), the posteriors contain significantly more information than the priors.
%}\label{fig:SOBHPowerRidge}
%\end{figure}

%\subsection{Restricted Inference on Relative Abundance}\label{sec:mixingFractionInference}

%\begin{figure*}
%\includegraphics[width=.48\linewidth]{PBHPopFractionRidgeFixedModelComparison.pdf}
%\includegraphics[width=.48\linewidth]{SOBHPopFractionRidgeFixedModelComparison.pdf}
%\caption{
%	Shown above are the posterior distributions on the relative abundance for the PBH (left) and SOBH (right) subpopulations, for both the full analysis and the restricted analysis plotted as the shaded region and the hatched region, respectively.
	%The prior for the mixing fractions in the case of the restricted analysis was a broad Dirichlet distribution.
	%There is good agreement between the two methods in the absence of systematic effects, as the true distributions of each %subpopulation are assumed to be those of the injection for the restricted analysis.
%}\label{fig:PopFractionRidgeFixedModelComparison}
%\end{figure*}


%%We now move onto the restricted analysis (Sec.~\ref{sec:populations}) where distributions in $t_E$-$\pi_E$ space are fixed to match those that created the data, and we only infer the relative relative abundances of each subpopulation. While more restricted in flexibility (as discussed in the following section), this comes at the benefit of $\approx10^{2}$ computational speed up.\footnote{The full population inference takes approximately 360 CPU hours on cluster-grade Intel Xeon E5-2695 nodes, and the restricted analysis takes approximately 1 CPU hour on a consumer-grade Intel Core i9-9980HK chip.} Fig.~\ref{fig:PopFractionRidgeFixedModelComparison} shows the posterior constraints abundances of the PBH and SOBH subpopulations compared with the full population model used in Sec.~\ref{sec:generalPopResults}. We see good agreement between the two analyses, with constraints being tighter in the restricted model due its comparative lack of flexibility. This significantly more computationally efficient restricted analysis gives unbiased and similar constraints on the abundances to the full analysis when we condition on knowing the model that generated the data, however, it has to be validated in a more realistic setting before fully adopted. 

%In addition to the full analysis performed above, we proposed a restricted analysis concerned only with the relative abundances in Sec.~\ref{sec:populations}.
%In this analysis distributions in $t_E$-$\pi_E$ space are fixed to match those that created the data, and the only inferred parameters are the relative heights of each distribution.
%This method produces posterior distributions on the relative abundances shown in Fig.~\ref{fig:PopFractionRidgeFixedModelComparison} for the PBH and SOBH subpopulations.
%For reference, the posterior calculated from the full analysis is shown in the same figure (from Sec.~\ref{sec:generalPopResults}).

%We see good agreement between the two methods, lending confidence to our results.
%The constraints are tighter in the restricted analysis, as expected due to the lack of flexibility.
%However, the results are unbiased and offer a comparable error bar on the parameters of interest.
%When conditioning this method on the true distributions that created the data, this analysis provides a significantly more computationally efficient analysis with very similar results. 
%However, this conclusion will require further validation as systematic effects in the shapes of the population distributions have been totally disregarded.

%\begin{figure}
%\includegraphics[width=\linewidth]{massRidgeIndividualPopFixedModelSystematics.pdf}
%\caption{
%	Shown above are the mass distributions for the different data sets assumed while re-conducting the restricted analysis.
%	The true distributions are the models used to generate the data (shown as a solid black line for each set of data), while the models used to re-apply the analysis are shown as a dashed black line.
	%The biased mass distributions for each subpopulation are shown as well, where the stellar subpopulation is represented %by a green dotted line, the SOBH subpopulation is represented by a orange dash-dotted line, and the PBH subpopulation is %represented by a purple dash dotted line. 
%    Each subpopulation distribution is normalized independently, so the relative heights do not reflect the total population.
%	These mass distributions used to re-conduct this analysis were chosen by finding the $90$-th percentile of the posterior %of the full analysis.
%}\label{fig:massRidgeFixedModelSystematics}
%\end{figure}

%To investigate the sensitivity of the restricted analysis to biased assumptions about the underlying population, we take $10$-th percentile posterior sample from the full three subpopulation model for $\hyp_{0-4}$ and run the restricted analysis with an alternate assumption for the underlying form of the mass spectra. This procedure injects bias into our analysis which simulates not knowing the subpopulation models exactly. While any number of alternative mass spectra could have been picked, we chose distributions that were different from the truth while still being consistent with the data in $t_E$-$\pi_E$ space. Fig.~\ref{fig:massRidgeFixedModelSystematics} shows the alternative mass spectra along the true spectrum used to generate the data.

%Fig.~\ref{fig:PopFractionRidgeFixedModelComparisonSystematics} shows the posterior constraints on the PBH and SOBH abundances using the restricted model, both assuming an unbiased and the new, biased population model. The general disagreement between these posteriors highlights the fact that biased modeling assumptions can impact the conclusions drawn with the restricted model. While the posteriors do overlap in each case, there is clear systematic bias, larger than the statistical error, that can lead to incorrect conclusions. Each of the biases can be connected with features in the assumed mass distribution. 
%For example, for $\hyp_4$, we see that the stellar population in our assumed model is more peaked than the true distribution, leading to posteriors for both the PBH and SOBH relative abundances which are biased high, compensating for the lack of support at higher mass from the stellar population. Finally, Fig.~\ref{fig:massReconstructionFixedModelSystematics} shows the effect on the mass reconstruction assuming incorrect distributions for each subpopulation. The biased reconstructions favor biased mixing ratios to compensate for the systematics in the shape parameters between the true distribution and the assumed ones.

%To provide some initial assessment of this issue of systematics and its impact on our results, we can rerun our analysis with an alternate assumption for the underlying distribution for each population (artifically injecting bias).
%From the posterior distributions of the full analysis, we calculated the $90$-th percentile and recorded the corresponding parameters of the mass distribution.
%We then used this model as the basis for our restricted analysis.
%While any number of incorrect distributions could have been picked, we chose these particular models as they are quite different from the true distributions for the mass while still being moderately consistent with the data in $t_E$-$\pi_E$ space.
%These distributions are shown in Fig.~\ref{fig:massRidgeFixedModelSystematics}, where we plot the true distribution actually used to generate the data, the total biased distribution used to conduct this second analysis, and the components of that biased distribution, separated by subpopulation.
%For concreteness, each of these biased distributions might simply represent a simulation of our Milky Way with different assumptions about the physics, a very realistic situation given our uncertainty of the SOBH and PBH population in particular.


%\begin{figure*}
%\includegraphics[width=.48\linewidth]{PBHPopFractionRidgeFixedModelComparisonSystematics.pdf}
%\includegraphics[width=.48\linewidth]{SOBHPopFractionRidgeFixedModelComparisonSystematics.pdf}
%\caption{
%	Shown above are the posterior distributions on the relative abundance for the PBH (left) and SOBH (right) subpopulation, for both the unbiased restricted analysis using the correct distribution (unhatched) and a systematically biased restricted analysis (hatched).
	%The assumed mass distributions for the biased analysis are shown in Fig.~\ref{fig:massRidgeFixedModelSystematics}.
	%The prior for the mixing fractions in the case of the restricted analysis was a broad Dirichlet distribution.
	%While the conclusions are mildly consistent, a clear systematic bias can be seen in the posteriors that suggests caution %should be exercised when applying this methodology.
%}\label{fig:PopFractionRidgeFixedModelComparisonSystematics}
%\end{figure*}

%Re-conducting the restricted analysis with our biased distributions produced posteriors on the relative abundances shown in Fig.~\ref{fig:PopFractionRidgeFixedModelComparisonSystematics} for the PBH and SOBH abundances. 
%We have plotted both the original posteriors using the unbiased distributions (unhatched) and the new, biased results (hatched).
%There is reasonable concern about biased modeling assumptions impacting the conclusions in this study.

%While the posteriors do overlap in each case, there is clear systematic bias, larger than the statistical error, that can lead to incorrect conclusions.
%Each of the biases can be connected with particular features in the assumed mass distribution. 
%For example, in the case of $\hyp_4$, we see that the stellar population in our assumed model is more peaked than the true distribution, leading to posteriors for both the PBH and SOBH relative %abundances to be biased high, compensating for the lack of support at higher mass from the stellar population.

%Finally, we can see the effect in the mass reconstruction of assuming incorrect distributions for each subpopulation, shown in Fig.~\ref{fig:massReconstructionFixedModelSystematics}.
%In this figure, the biased reconstructions (hatched) favor biased mixing ratios to compensate for the systematics in the shape parameters between the true distribution and the assumed ones.
%Compared with the unbiased reconstruction (unhatched), the biases 

%The inference from the restricted model suggests that it could provide a computationally fast and tractable alternative to the full model inference if the form of the population mass spectra is relatively well known \emph{a priori}. However, in the current realistic case that the population model is not well known, the restricted analysis could lead to biased conclusions. The full method of Sec.~\ref{sec:generalPopResults} can be extended to robustly marginalize over any reasonable population uncertainty and should be the default method for performing hierarchical inference until the lens population mass spectrum is better understood.



%Once there is more understanding about the underlying population models, this restricted method could be a tractable alternative allowing one to quickly measure abundances.
%However, our initial exploration of the systematics when using the restricted model emphasizes the need to utilize the full method (Sec.~\ref{sec:generalPopResults}) until the %uncertainties in the underlying distributions are relatively under control.
%The full method of Sec.~\ref{sec:generalPopResults} can be extended to robustly marginalize over any reasonable population uncertainty and should be the \emph{de facto} method %for performing hierarchical inference for the near future.
%The biases observed in our work are also a testament to the danger of making hard assumptions about populations of lenses and fixing hyperparameters to unique values.
%Without accounting for the uncertainties in a robust way (i.e., through marginalization or some other process), there is real danger in arriving at systematically biased %conclusions.

%\begin{figure}
%\includegraphics[width=\linewidth]{massReconstructionRidgeFixedModelSystematics.pdf}
%\caption{
%	The reconstruction of the mass distribution of the entire lens population from the posterior of the restricted analysis using the true underlying distributions (unbiased, non-hatched and green) and systematically biased assumptions (biased, hatched and orange). 
%	The actual distributions are shown in black as dashed lines.
%	We can see that the relative abundances favor biased values to compensate for systematics in the shapes of the %distributions for each subpopulation.
%}\label{fig:massReconstructionFixedModelSystematics}
%\end{figure}

%The methods of this work outperformed current strategies being used to classify lenses in search of BH candidates, with accompanying uncertainty quantification and the possibility of marginalizing over population uncertainty.
%On top of individual event classification, our analysis revealed the structure of intrinsic uncertainty due to degeneracies in the population model (independent of measurement accuracy). 
%Applying the methods proposed here and incorporating this information about regions in event parameter space fundamentally more or less uncertain can help with accurately and efficiently looking for BH candidates for astrometric follow-up.

%For hierarchical inference, the full method (used to infer both the structure of mass distributions and relative abundance of different subpopulations of lenses) leads to inference that is accurate and effective while appropriately handling population uncertainty.
%In the context of characterizing a PBH subpopulation of lenses in our synthetic data, we have shown that our methodology has potential to shed light on this anomalous subpopulation of lenses.
%In particular, we find the posterior distribution on the relative abundance is almost entirely inconsistent with zero when considering the unrealistic situation where PBHs account for $100\%$ of DM.
%In more realistic scenarios where PBHs account for at most $\sim 25\%$ of DM, our ability to identify the subpopulation begins to deteriorate, and we are only capable of placing upper limits on the subpopulation.
%These results are derived through a rigorous analysis of the different products of the hierarchical method, built on maximum likelihood measurements, Bayes' factors, and hyperparameter posteriors.
%While the simulations are somewhat simplistic, they capture many of the critical features present when analyzing real data.

%Furthermore, inference about less exotic physics was also achievable.
%Certain combinations of hyperparameters and the relative abundances of stellar and SOBH lenses were measurable, although the success of these methods depended on the particular data set.
%In the case of stellar lenses, the conclusions were largely independent of the number of BHs in the data, as stellar lenses vastly outnumbered the BH lenses.
%However, in the case of the SOBH lenses, inference about the slope of the powerlaw distribution and the relative abundance were measurable if not considering a PBH subpopulation, but the degeneracies %between SOBH and PBH populations made it difficult to disentangle the two when simultaneously fitting for both subpopulations.

%However, other features of the population model (like the minimum SOBH mass) were inaccessible with these methods, given our simulated data, illustrating that some science targets require a more refined analysis. 
%This can either come through increased volume of data (through larger and/or longer surveys), increased measurement precision or the incorporation of heterogeneous data (such as astrometric information). 
%Characterizing what exactly would be required to measure this feature of the mass distribution is left to future work.

%As part of the methods proposed in this work, a computationally efficient restricted hierarchical framework was also introduced.
%hile making more restrictive assumptions (that the various shapes of the mass distributions of each subpopulation were fixed), the approximately $10^2-10^3$ improvement to computational performance can be a powerful tool in rapid hierarchical inference.
%When conditioning on the true hyperparameters of the mass distributions, we see good agreement between the full method and the restricted one.
%Unfortunately, we see from this initial validation that the method is moderately susceptible to systematic bias if biased distributions are assumed instead of the true ones. 
%Given current uncertainty on population modeling, we recommend the full analysis be implemented for hierarchical studies until %the population models are better understood.

%%%%%%%%%%%%%%%%%%%%%% OLD text %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%In this work, we have extended and applied established methodology to the problem of inferring the mass distribution of lensing objects in the Milky Way through extensive simulation.
%%We outlined and validated the appropriate method for accounting for noisy measurements and selection effects into hierarchical inference for astronomical data, building off and extending past work to apply these methods to searches for PBHs in photometric microlensing surveys.
%This involved the analysis of single events in the context of their parent populations (Sec.~\ref{sec:singleEventClass}) and the full hierarchical analysis described in (Sec.~\ref{sec:stats}).
%We then validated and verified our methodology by simulating several microlensing surveys, involving thousands of microlensing events and analogous to the sensitivity and duration of existing microlensing surveys.
%We calculated the full posterior for each event using the fully robust technique of MCMC sampling.
%With several different realizations, we then performed our hierarchical and individual event analyses, providing a suite of metrics and predictions for the efficacy and accuracy of our methods.
%
%From these simulations, we determined that this method has competitive abilities to measure certain features of the mass distribution, including the slope of the powerlaw distribution for the SOBH and stellar populations, as well as measuring other key features of the stellar subpopulation (the largest subpopulation by a wide margin).
%We also find our methods are competitive at placing constraints on the fraction of DM that can be comprised of an undetected PBH subpopulation, possibly providing evidence for such a subpopulation (given enough ``signal'' in the data).
%In the absence of PBHs in the data, we find that we can place a rigorous upper limit to the fraction of DM that could possibly be made up of a PBH subpopulation, robustly accounting for population model uncertainties.
%However, not all open science questions are answerable with this data and this set of techniques.
%Probes of the mass gap between NSs and BHs is most likely out of reach of this methodology, assuming photometric only, OGLE-type data.
%This conclusion may change with future surveys or joint astrometric observation.
%
%When using our restricted hierarchical analysis, we see promising results \emph{when conditioning on the true, underlying distribution hyperparameters}.
%Re-conducting the analysis with large systematic bias in these assumptions showed concerning disagreement between the two analysis.
%This suggests that the full analysis be used for the near future until further work helps to restrict the range of population models to a reasonable range.
%
%We also presented results on understanding the individual events in the context of their parent populations.
%We showed that the method has promise in categorizing a few, well measured events, but is also susceptible to systematic bias if the uncertainty of the population model is not taken into account.
%For a vast majority of events, however, the inference about the individual lenses was uninformative in disentangling the lens' true nature.
%Again, these results speak to the need for marginalization and to be cautious when assuming lenses belong to a certain subpopulation (particularly when only using photometric data).
%
%Future avenues of research include in-depth analysis of the robustness of these methods to systematic errors in the modeling.
%Incorrect assumptions about the input physics will no doubt impact our conclusions, but at what point are the systematics greater than the statistical error?
%More dimensions of the hyperparameter space could help extract information about the subpopulations.
%For example, integrating the blending fraction, velocity distribution and spatial distributions of lensing objects into the analysis can help disentangle the different subpopulations, potentially providing stronger conclusions about the underlying astrophysics.
%Yet the additional flexibility, if not warranted and too degenerate with other model components, might degrade the effectiveness of this methodology.
%Furthermore, reliable and tractable population forward modeling will need to be implemented before applying these methods to actual data.
%At the moment, our toy problem relied on analytic distributions for the various event parameters, however, the real data will no doubt be described by much more complicated, non-analytic distributions requiring full simulation by software like {\tt PopSyCLE}.

\begin{comment}
Until now, we have have remained largely agnostic about the details of the data or statistical model (with the caveat of the assumptions outlined throughout, such as stationary noise, no background events, etc.), but now we assign an actual joint likelihood function to the event parameters and detection number distribution, $p(\{\eparamdi\}, \{\eparamndj\}, \NOBS, \NNOBS, \NNOEVENT| \hyp)$.
First, we will assume independence between datasets. 
However, we will assume the rate is common to all signals and is uniform in time but dependent on event parameters.
We will take advantage of the following reparametrization of the differential rate for the number of events $N$ for some population,
\begin{equation}
\frac{d N }{d \eparam}(\eparam|\hyp) = N(\hyp) p(\eparam | \hyp) \,.
\end{equation}

Considering these details (statistical independence of counts with a nonuniform rate), we will model the event rates as an inhomogeneous Poisson process~\citep[e.g.,][]{gregory_2005,2011ApJ...742...38Y,Loredo:2004,2011ApJ...742...38Y}.
To derive this from these two assumptions, we start by dividing our parameter space into bins of size $\delta \eparam$. 
If we consider each bin independently, we would expect a homogeneous Poisson process to predict the number of counts in that bin, $n_l(\hyp)$ for $l \in (0,N_{\rm bins})$ and $N_{\rm bins}$ number of bins.
The counts will be a function of the population model and its parameters, $\hyp$.
The expected rate count in a given bin is calculated as 
\begin{equation}\label{eq:binIntegral}
n_l(\hyp) = \int_{\delta \eparaml} \frac{d N}{d \eparam}(\eparam| \hyp) d\eparam \,.
\end{equation}
This yields the overall likelihood of actually observing $\{n_{l,{\rm data}}\}$ counts in each bin
\begin{equation}
p(\{n_{l,{\rm data}}\} | \hyp) =\prod_l^{N_{\rm bins}} \frac{(n_l(\hyp))^{n_{l,{\rm data}}} e^{-n_l(\hyp)}}{n_{l, {\rm data}}!} \,.
\end{equation}

Now, we can take the limit $\delta \eparam $ being very small, such that that we find that all the bins either contain a single observed event ($n_{l,{\rm data}}=1$) or no event ($n_{l,{\rm data}}=0$) and the rate is approximately constant across the range.
%\sepc{This didn't make sense at first to me, but now it's the best derivation I can think of.. The reason we make this approximation is so that the likelihood factorizes as a product of independent detections while incorporating (inhomogeneous) Poisson statistics.}
%\sepc{This didn't make sense at first to me, but now it's the best derivation I can think of.. It's just a pretty common trick to exchange the integral in Eq.~\ref{eq:binIntegral} into a product of the rate and a constant bin width, which falls out or is reabsorbed in the evidence. This isn't really a statement about what we can observe, but about how to extend a Poisson distribution to be parameter dependent (more of a mathematical statement). Assuming the function is well behaved, we can always find a discretization that satisfies this.}
In the continuous limit, the bin identification corresponds to a specific set of event model parameters, $\eparaml$.
This means that in lieu of using subscripts $l$ to denote the bin (and therefore the parameters), we can write this as a continuous function $n(\eparaml|\hyp)$ given by 
\begin{equation}
n_{l} \rightarrow n(\eparaml|\hyp) = \frac{d N}{d \eparam}(\eparaml | \hyp)  \delta \eparam = N(\hyp) p(\eparaml | \hyp) \delta \eparam\,.
\end{equation}
This allows us to now exchange our observable from the observed counts per bin $n_{l,{\rm data}}$ to the observed parameters $\eparaml$, which we assume are measured perfectly for this step of the calculation.
Uncertainty in these parameters are encoded through the likelihood, which will be reintroduced below.
Bins with zero events will contribute a factor of 
\begin{equation} 
e^{-n(\eparaml|\hyp)}\,,
\end{equation} 
and bins with an event will contribute
\begin{equation} 
n(\eparaml|\hyp) e^{-n(\eparaml|\hyp)}\,.
\end{equation} 
Now we can consider $\Nt$ events with $\{\eparamdi\}$ parameters, $i\in [0,\Nt]$, detected or not.
This gives the following distribution for the observed parameters
\begin{equation}
p(\{\eparamdi\}, \Nt| \hyp) = e^{-N(\hyp)} \prod_l^{\Nt} n(\eparamdi|\hyp)\,,
\end{equation}
where $N(\hyp) = \int d\eparam \frac{d N }{d \eparam}(\eparam| \hyp)\approx \sum_l n(\eparaml| \hyp)  $. 
We note that the sum is over \emph{bins} when defining $N(\hyp)$, not the events. 
That is because every bin contributes to the sum in the exponential, but the product only spans the events that actually occur.

Here, we note that if we were to marginalize over $\Nt$ and $\{\eparamdi\}$, this likelihood is not normalized.
Normally, this does not present an issue, as the normalization constant does not matter in most sampling algorithms. 
However, as we will see in the next step, it is important when marginalizing over variables.
Therefore, to ensure this likelihood is normalized, we can divide by $\Nt!$. 
%To verify our likelihood is now normalized, we can explicitly compute the integral and summation
%\begin{align}\nonumber
%\sum_{\Nt = 0}^{\infty} \int d \{\eparamdi\} p(\{\eparamdi\}, \Nt | \hyp) &= \sum_{\Nt = 0}^{\infty} \int d \{\eparamdi\} \frac{e^{-N(\hyp)}}{\Nt !} \prod_l^{\Nt} n(\eparamdi|\hyp)\,, \\
%&= 1\,.
%\end{align}

\end{comment}

% Take 2
%Gravitational microlensing offers a novel window into the dark universe that no other observable currently can: the observation of \emph{isolated and dark} compact objects.
%%All other probes of dark compact objects in our universe depend on interactions between the black hole and its environment or a companion.  
%However, studying and identifying candidate BH lenses must address known issues like degeneracies in both the event modeling parameters themselves and in their predicted distributions from models of different subpopulations of lenses.
%%Past work has addressed these problems by making cuts to the data based on observable parameters and comparing observables to distributions based on galactic and stellar models.
%In this work, new methods are proposed that extend past work to better address these issues and uncertainties, including a method to probabilstically identify BH lenses and two methods to infer population hyperparameters through hierarchical inference, where one is more flexible and the other is more computational tractable.
%%These methods are validated by simulating multiple populations of microlensing events (including hypothetical primordial black hole lenses) with accompanying ground-based survey then inferring the characteristics of the population as a whole.
%These methods are validated by simulating multiple microlensing event populations with accompanying ground-based survey then inferring the characteristics of the population as a whole. 
%In particular, the characterization of a hypothetical population of primordial black holes is evaluated.
%%The methods proposed here outperform examples of current BH lens identification pipelines (in terms of the purity of the candidates identified) while also naturally including uncertainty estimates and uncertainty marginalization.
%The methods proposed here outperform examples of current BH lens identification pipelines in terms of the purity of the candidates identified, while also naturally including uncertainty estimates and uncertainty marginalization.
%The fully flexible hierarchical method robustly infers things like the relative abundances of different subpopulations of lenses, and in the case of primordial black holes, can potentially place constraints on its abundance comparable to existing microlensing results.
%However, it fails to capture certain nuanced features in the data like the existence of a mass gap between BHs and other stellar lenses, at least while considering current photometric precision.
%The restricted hierarchical analysis, which is conditioned on knowing certain features of the population model \emph{a priori}, performs well when the correct assumptions are made, but fails to recover unbiased estimates of population hyperparameters when using incorrect assumptions about the underlying populations. 
%This suggests the more flexible model be used until the population of lenses is better understood.

%\sepc{Trying again above}

%Gravitational microlensing offers a novel window into the dark universe that no other observable currently can: the observation of \emph{isolated and dark} compact objects.
%All other probes of dark compact objects in our universe depend on interactions between the black hole and its environment or a companion.  
%Microlensing only relies on the warping of the light from background stars by intervening massive objects. 
%This fact allows microlensing surveys to be sensitive to large segments of the black hole population inaccessible through other means.
%%Large catalogs of microlensing observations can shed light on the population of isolated compact objects through these indirect observational techniques.
%%Many probes exist that can shed light on the underlying population of compact objects in our universe, but they depend on the strong interaction between the compact object and its surroundings through the emission of gravitational waves or through the accretion of matter onto the compact object itself.
%%Meanwhile, large catalogs of microlensing observations can be used to infer properties of the underlying population of isolated compact objects in our galaxy and even provide evidence for a particular object belonging to certain astrophysical populations, in some cases.
%%This type of observation does not come without its drawbacks, however, and care must be taken to properly account for the uncertainty in the measurements and other selection effects that this type of analysis can be susceptible to.
%In this work, we outline and extend both hierarchical and non-hierarchical statistical frameworks commonly utilized in many fields of astronomy. 
%We apply and adapt them for the context of microlensing data and mixture population models.
%%To validate this methodology, we run this analysis on a suite of different simulated catalogs of events, suggestive of current research related to black hole population science, early universe physics and cosmology.
%%To validate this methodology, we run this analysis on a suite of different simulated catalogs of events, suggestive of current research.
%To validate this methodology, we run these analyses on a suite of different simulated catalogs constructed to be suggestive of current research problems, in particular focusing on the detection of a subpopulation of primordial black holes as a component of dark matter.
%%In particular, we apply this methodology to the task of detecting a subpopulation of primordial black holes as a component of dark matter, as a proof of principle and a point of comparison for future research.
%%We find encouraging results for most of the other science cases we investigate in this work
%Our results suggest this can be a powerful method for the identification of individual events as belonging to the BH population or not, inferring the shape of the mass probability density function and relative abundance of lensing objects and identifying or constraining the subpopulation of primordial black holes in our galaxy, with varying effectiveness depending on the data being analyzed.
%However, we also find this method is not well suited for addressing some problems, such as the measurement of a mass-gap between neutron stars and black holes, .
%This work lays the foundation for the application of this framework to current and future surveys (both microlensing and general), yielding deep insights into astrophysical populations of all types.
%end-include
